Parallel Monte Carlo Tree Search with Batched Rigid-body Simulations for Speeding up Long-Horizon Episodic Robot Planning

We propose a novel Parallel Monte Carlo tree search with Batched Simulations (PMBS) algorithm for accelerating long-horizon, episodic robotic planning tasks. Monte Carlo tree search (MCTS) is an effective heuristic search algorithm for solving episodic decision-making problems whose underlying search spaces are expansive. Leveraging a GPU-based large-scale simulator, PMBS introduces massive parallelism into MCTS for solving planning tasks through the batched execution of a large number of concurrent simulations, which allows for more efficient and accurate evaluations of the expected cost-to-go over large action spaces. When applied to the challenging manipulation tasks of object retrieval from clutter, PMBS achieves a speedup of over $30\times$ with an improved solution quality, in comparison to a serial MCTS implementation. We show that PMBS can be directly applied to real robot hardware with negligible sim-to-real differences. Supplementary material, including video, can be found at https://github.com/arc-l/pmbs.

==> texs/app.tex <==
\subsection{Grasp Classifier Implementation Details}
For our implementation of the grasp classifier (GC), we used Isaac Gym to collect grasp training data.
%
Random objects are first sampled on the workspace, and then we discretize the workspace into a grid, where each point is the $(x,y)$ of a grasp action $a^g$.
We also discretize rotation into $K$ angles uniformly.
All robots in simulator will pick one grasp action and check the distance between two fingers as a signal of successful grasping.
For each depth image, it is associated with hundreds of grasps. If the target can be grasped in at least $n$ attempts, then the label is 1, and 0 otherwise ($n$ = 5).
We used two days of generating 20000 training data (a depth image focus centered on the target object and a label of can it be grasped) without human annotation.
It is evaluated on test data with $93.45\%$ accuracy if the $R_c^{*}$ equals 0.7.
The batch size is $256$, learning rate is $0.1$, epochs is $90$, momentum is $0.9$.
We have successfully reduced the grasp evaluation time from $0.26$ to $0.003$ per image, making the parallel MCTS possible.


